A new family of $2$-scattered subspaces and related MRD codes

Scattered subspaces and $h$-scattered subspaces have been extensively studied in recent decades for both theoretical purposes and their connections to various applications. While numerous constructions of scattered subspaces exist, relatively few are known about $h$-scattered subspaces with $h\geq2$. In this paper, we establish the existence of maximum $2$-scattered $\F_q$-subspaces in $V(r,q^6)$ whenever $r\geq 3$, $r\ne 5$, and $q$ is an odd power of $2$. Additionally, we explore the corresponding MRD codes.

==> openprob.tex <==
\subsection*{Open Problem}
 A set $S\subseteq \PG(k-1,q^m)$ is called \emph{$\rho$-saturating} if every point of $\PG(k-1,q^m)$ lies in a subspace generated by $\rho+1$ points of $S$. The above definition comes from \cite{pamb}. By MAGMA calculations we obtained that when $q=2$, $U$ is $2$-saturating. It would be interesting the study of such property for any odd power of $2$.
